Balanced Datasets Are Not Enough: Estimating and Mitigating Gender Bias in Deep Image Representations

In this work, we present a framework to measure and mitigate intrinsic biases with respect to protected variables --such as gender-- in visual recognition tasks. We show that trained models significantly amplify the association of target labels with gender beyond what one would expect from biased datasets. Surprisingly, we show that even when datasets are balanced such that each label co-occurs equally with each gender, learned models amplify the association between labels and gender, as much as if data had not been balanced! To mitigate this, we adopt an adversarial approach to remove unwanted features corresponding to protected variables from intermediate representations in a deep neural network -- and provide a detailed analysis of its effectiveness. Experiments on two datasets: the COCO dataset (objects), and the imSitu dataset (actions), show reductions in gender bias amplification while maintaining most of the accuracy of the original models.

==> sections/setup.tex <==
We consider two datasets.
First, the COCO dataset~\cite{lin2014microsoft}, consisting of images annotated with objects corresponding to $80$ categories, and $5$ textual descriptions for each image.
In this dataset we perform multi-label object classification.
Additionally we adopt the imSitu dataset~\cite{yatskar2016} where each image is annotated with a structured tuple consisting the name of an activity (a verb) and the participants in the activity (roles). 
In this dataset, we perform activity recognition in the form of a multi-class classification task.

\paragraph{Datasets} This paper follows the setup of existing work for studying bias in COCO and imSitu~\cite{zhao2017men}.
In COCO, we examine object classification. We use image captions from COCO as a proxy for annotations of gender of the main entity in the image: an image is considered ``male'' if the word ``man'' is present in the caption or ``female'' if word ``woman'' is in the caption. 
In imSitu, we consider situations (activities are annotated in addition to objects and semantics roles, a classification of how objects are participating in activities).
We say an image is ``male'' if we can find the word ``man'' in the gloss of the ``agent'' of an activity and female if we can find the word ``woman'' in the gloss. 
Finally, for the purpose of our analysis, we exclude ``person'' category from COCO $80$ categories.
For imSitu, we filter non-human oriented activity categories following \cite{zhao2017men}. For both COCO and imSitu, we further exclude extremely imbalanced categories that only appear with ``man'' or ``woman'', resulting $79$ objects and $211$ activities. We ensure every image contains at least one target category. Thus, we have $22,826$ images for training, $5,367$ for validation and $5,473$ for test from COCO. Similarly, there are $24,301$ training images, $7,730$ validation images and $7,669$ test images from imSitu.

\paragraph{Models}
For both COCO object classification and imSitu activity recognition, we use a standard ResNet-50 convolutional neural network pretrained on Imagenet (ILSVRC) as the underlying model by replacing the last linear layer as appropriate.
When constructing attackers, we use a 4-layer multi-layer perceptron (MLP) with BatchNorm and LeakyReLU in between for both dataset and model leakage estimates.


\paragraph{Metrics}
We evaluate using mAP, or the mean across categories of the area under the precision-recall curve, and F1 for both object and activity classification by using the discrete output predictions of the model.

\paragraph{Leakage Computing}Prediction leakage was predicted from pre-activation logits while dataset leakage was predicted from binary labels.
Attackers were trained and evaluated on an equal quantity of male and female images, sampled from the original development and test sets. Note we do not touch the training data used to train the model because the model has seen both images and ground truths and thus may perform differently.
To train an attacker on COCO, we randomly sample $500$ male images and $500$ female imags from the original development set as training data. And we randomly sample $250$ male images and $250$ female images from the original test set as dev and test respectively. For imSitu, we randomly sample $2,000$ male images and $2,000$ female images for training, and $1,000$ male and $1,000$ female images as dev and test set respectively.
% We need to do randomling sampling 5 times.
We run $10$ rounds and report the averaged accuracy on the test set as the leakage score.

\paragraph{Training Details}
For comparability, all models are developed and evaluated on dev and test sets from the original data (even when we modify the composition of a training set). We load weights from a ResNet-50 pretrained on ImageNet and optimize using Adam~\cite{Adam} with a learning rate of $1e-4$ and a minibatch size of $32$ for training the linear layers for classification. We then fine-tune the model with a learning rate of $5e-6$. 
In adversarial training, we always first train linear layers for classification with $5e-5$ learning rate and batch size $64$ until the performance plateaus.
We incorporate adversarial training when we fine-tune the model end to end using a learning rate $1e-5$.
Before we start adversarial training, we first train the gender classification branch so that its gradients provide useful guidance for feature removal during adversarial training.
We train all attackers for $100$ epochs with a fixed learning rate of $5e-5$ and a batch size of $128$, keeping the snapshot that performs best on the dev set.
As training data is not always gender balanced, we sample the same amount of male and female images in every batch to encourage the gender classifier focus on gender features.

